Estimation-Throughput Tradeoff for Underlay Cognitive Radio Systems

Understanding the performance of cognitive radio systems is of great interest. To perform dynamic spectrum access, different paradigms are conceptualized in the literature. Of these, Underlay System (US) has caught much attention in the recent past. According to US, a power control mechanism is employed at the Secondary Transmitter (ST) to constrain the interference at the Primary Receiver (PR) below a certain threshold. However, it requires the knowledge of channel towards PR at the ST. This knowledge can be obtained by estimating the received power, assuming a beacon or a pilot channel transmission by the PR. This estimation is never perfect, hence the induced error may distort the true performance of the US. Motivated by this fact, we propose a novel model that captures the effect of channel estimation errors on the performance of the system. More specifically, we characterize the performance of the US in terms of the estimation-throughput tradeoff. Furthermore, we determine the maximum achievable throughput for the secondary link. Based on numerical analysis, it is shown that the conventional model overestimates the performance of the US.

==> figures/fig_P_f_vs_est_time_diff_snr_AWGN.tex <==
% This file is generated by the MATLAB m-file laprint.m. It can be included
% into LaTeX documents using the packages graphicx, color and psfrag.
% It is accompanied by a postscript file. A sample LaTeX file is:
%    \documentclass{article}\usepackage{graphicx,color,psfrag}
%    \begin{document}\input{fig_P_f_vs_est_time_diff_snr_AWGN}\end{document}
% See http://www.mathworks.de/matlabcentral/fileexchange/loadFile.do?objectId=4638
% for recent versions of laprint.m.
%
% created by:           LaPrint version 3.16 (13.9.2004)
% created on:           03-Feb-2015 17:20:02
% eps bounding box:     24 cm x 18 cm
% comment:              
%
%\begin{psfrags}%
%\psfragscanon%
%
% text strings:
\psfrag{s01}[b][b]{\color[rgb]{0,0,0}\setlength{\tabcolsep}{0pt}\begin{tabular}{c}$\pfa$\end{tabular}}%
\psfrag{s02}[t][t]{\color[rgb]{0,0,0}\setlength{\tabcolsep}{0pt}\begin{tabular}{c}$\test$ = [ms]\end{tabular}}%
\psfrag{s06}[][]{\color[rgb]{0,0,0}\setlength{\tabcolsep}{0pt}\begin{tabular}{c} \end{tabular}}%
\psfrag{s07}[][]{\color[rgb]{0,0,0}\setlength{\tabcolsep}{0pt}\begin{tabular}{c} \end{tabular}}%
\psfrag{s08}[l][l]{\color[rgb]{0,0,0}pfal}%
\psfrag{s09}[l][l]{\color[rgb]{0,0,0}pfap}%
\psfrag{s10}[l][l]{\color[rgb]{0,0,0}pfau}%
\psfrag{s11}[l][l]{\color[rgb]{0,0,0}pfal}%
%
% xticklabels:
\psfrag{x01}[t][t]{2}%
\psfrag{x02}[t][t]{4}%
\psfrag{x03}[t][t]{6}%
\psfrag{x04}[t][t]{8}%
\psfrag{x05}[t][t]{10}%
\psfrag{x06}[t][t]{12}%
\psfrag{x07}[t][t]{14}%
%
% yticklabels:
\psfrag{v01}[r][r]{$10^{-4}$}%
\psfrag{v02}[r][r]{$10^{-3}$}%
\psfrag{v03}[r][r]{$10^{-2}$}%
\psfrag{v04}[r][r]{$10^{-1}$}%
%
% Figure:
%\resizebox{12cm}{!}{\includegraphics{fig_P_f_vs_est_time_diff_snr_AWGN.eps}}%
%\end{psfrags}%
%
% End fig_P_f_vs_est_time_diff_snr_AWGN.tex

